Space Networking Kit: A Novel Simulation Platform for Emerging LEO Mega-constellations

This paper presents SNK, a novel simulation platform designed to evaluate the network performance of constellation systems for global Internet services. SNK offers realtime communication visualization and supports the simulation of routing between edge node of network. The platform enables the evaluation of routing and network performance metrics such as latency, stretch, network capacity, and throughput under different network structures and density. The effectiveness of SNK is demonstrated through various simulation cases, including the routing between fixed edge stations or mobile edge stations and analysis of space network structures.

==> data/model.tex <==
\section{System Model}


% \input{tab/symbols.tex}

% \textbf{\textit{Definition 1:}}%time
\subsection{Network Model}

To tackle the temporal variations in the satellite networks,
we denote an ordered time set as $ \mathcal{T}= \{t_1, t_2,\cdots \}$.
% The elements of the set $\mathcal{T}$ are called time stamps, where $t_i \le t_{i+1}$.
The network topology without eISLs can be considered unchanged between
adjacent time stamps. $t_{i+1}- t_i$ represents the minimum time granularity of scenario change.
% and the time granularity with each element represent one second of time can be simply described as a time set $\mathcal{T} = \{1, 2, T\}$. 
Then, the network topology at each time stamp
$t \in \mathcal{T}$ can be formulated as an undirected graph $\mathcal{G}^t = (\mathcal{V},\mathcal{E}^t )$, where $\mathcal{V}$ is the set of network vertices (satellites) and $\mathcal{E}^t$ is the set of undirected edges (feasible ISLs includes iISL, sISLs and eISLs).% intro部分就列好ISL种类

% \textbf{\textit{Definition 3:}} %Distance mat


% \textbf{\textit{Definition 4:}} %Visible mat
% \subsection{Visibility range and association range}
Let $\mathbf{r}^t(s_i)$ denote the column vector with the cartesian coordinates of satellite $s_i$ at time $t$. The Euclidean distance between two satellite $s_i, s_j$ is denoted as $d^t(s_i,s_j)$.
% The Earth blocks the line of sight (LoS) between two satellites $s_i$ and $s_j$ in orbital if $d^t(s_i,s_j) \geq LoS$, where $LoS$ is the maximum slant range (i.e., line-of-sight distance) between two arbitrary satellites. 
Assuming that the Earth is a perfect sphere, the line-of-sight (LoS) distance of two satellites is expressed as
\begin{eqnarray}
	LoS = 2 \sqrt{h^2 + 2hR_E }
\end{eqnarray}
where $R_E$ is the radius of Earth.
If $d^t(s_i,s_j) \ge LoS$, these two satellites $s_i$ and $s_j$ will be blocked by the Earth.
Hence, We define the visible matrix $\mathbf{V}^t = \{v^t_{ij}\}$.  $v_{ij}^t = 1$ if $d(s_i,s_j) \le LoS$ and $v_{ij}^t= 0$ if $d(s_i,s_j) \ge LoS$.
Futhermore, we define $d_\delta$ as the association range and $0 \leq d_\delta \leq LoS$, indicating that a eISL can be established if $d(s_i,s_j) \le d_\delta$ between satellites.
The association duration time is denoted as $T(s_i,s_j,d_\delta)$ which presents the duration time of $s_i,s_j$ within the association range.




% \textbf{\textit{Definition 5:}} %Matching mat
Let $m_{ij}^t \in \{0,1\}$ be the matching indicator that takes the value of 1 if a link between two satellites $s_i$ and $s_j$ is established at time $t$. 
% We use $g(s_i,s_j)$ to denote the constraint on whether a link can be established between two satellites; if the constraint is satisfied $g(s_i,s_j) = 1$, otherwise $g(s_i,s_j) =0$.
% \begin{eqnarray}
% 	m_{ij}^t =\left\{
% 		\begin{aligned}
% 		1& , & e_{ij} \in \mathcal{E}^t \\
% 		0 & , & e_{ij} \notin \mathcal{E}^t \\
% 		\end{aligned}
% 		\right.\\
% \end{eqnarray}
Furthermore, we assume that the iISL and sISL are persistent while eISL are time varying. The matching state can be formulated as a Matching Matrix
\begin{eqnarray}
\mathbf{M}_*^t = \mathbf{M}_{+} +\mathbf{M}_{-} + \mathbf{M}^t
\end{eqnarray}
where $\mathbf{M}_-, \mathbf{M}_+$ are constants to denote the adjacent state of iISL and sISL respectively, and $\mathbf{M}^t=\{m^t_{ij}\}$ describe whether a eISL exists between two satellites at time $t$. 
Then the topology of satellite network can be represented by a matching matrix $\mathbf{M}_*^{t}$ and is equivalent to the graph edge set $\mathcal{E}^t$ of $\mathcal{G}$.
The problem of building eISL can be transformed into a matching problem with the goal of finding a set of suitable $\mathbf{M}^t$ that maximizes a target value, subject to the constraints imposed by $\mathbf{M}_{+}$ and $\mathbf{M}_{-}$, which are fixed and given by the ISL building pattern.


% \textbf{\textit{Definition 5:}}% subject
% eISLs should not be established between some special satellites, such as coorbital satellites or satellites in near-orbit. we find that with the difference between $p(s_i)$ and $p(s_j)$ increase, the position of eISL (i.e. the center position of links) is increase, leading the high density of eISL in high latitude region while keep a lower utilization. Thus the constrains can be formulated as
% \textbf{\textit{Definition 6:}}% 
% \subsection{Topological distance}

To strike the balance between cost and connectivity, it is advisable to establish eISLs between topologically distant satellites whenever possible.
We define the minimum-hop between two satellites in the network without considering the eISL as the topological distance $g(s_i,s_j)$.
Let $\Delta p(s_i,s_j)$ denotes minimum-difference of satellite plane, which is given by
\begin{eqnarray}
	\Delta p(s_i,s_j) =\left\{
		\begin{aligned}
		&|p_i - p_j|, ~  \text{if}~|p_i - p_j| \leq P/2 ~\\
		&\mathop{min}\{p_i,p_j\}+P - \mathop{max}\{p_i,p_j\},~ else \\
		\end{aligned}
		\right.
\end{eqnarray}
where $p_i$ is the orbit plane number of $s_i$. Similarly, the phase difference is given by
\begin{eqnarray}
	\Delta f(s_i,s_j) =\left\{
		\begin{aligned}
		&|f_i - f_j|, ~  \text{if}~|f_i - f_j| \leq N_P/2\\
		&\mathop{min}\{f_i,f_j\}+N_P - \mathop{max}\{f_i,f_j\}  ,~ else \\
		\end{aligned}
		\right.\\
\end{eqnarray}
where the $N_P$ is the number of satellites per orbital-plane, and the $f_i$ is the phase number of $s_i$.
When the ID of satellite is known, the topological distance between two satellites can be found by using the following expression:
\begin{eqnarray}
	g(s_i,s_j) = \Delta p+ \Delta f
	\label{eq:hop1}
\end{eqnarray}
It is only for constellations with '+Grid' ISL pattern\cite{bhattacherjee2021towards}. The $g$ in '*Grid' ISL pattern should be
\begin{eqnarray}
	g(s_i,s_j) = \mathop{min}\{ \Delta p,\Delta f\} +	| \Delta p -\Delta f |
	\label{eq:hop2}
\end{eqnarray}

\subsection{Link Budget}
% \textbf{\textit{Definition 7:}}
At the time $t$, the received SNR at satellite $j$ from satellite $i$ is written as
\begin{eqnarray}
	\text{SNR}^t(s_i,s_j) = \frac{\text{EIRP} \cdot G_r}{k T_s  B_N L^t_f(s_i,s_j)}
\end{eqnarray}
where EIRP is the equivalent isotropically radiated power; 
$G_r$ is the receive antenna gains;
$k$ is Boltzmann’s constant; 
$T_s$ is the equivalent noise temperature in Kelvin;
and $B$ is the channel bandwidth in Hertz.
 $L_f$ is the Free Space Loss (FSL) which is given by $L^t_f(s_i,s_j) = (\frac{4 \pi d_{ij}^t}{\lambda})^2$ where $\lambda$ is the wave length of carrier signal.
Based on this expression, the data rates of the link between $s_i,s_j$ is formulated as link capacity, which is denoted as
\begin{eqnarray}
	R (s_i,s_j) = B \log_2 ( 1 + \text{SNR}(s_i,s_j)) 
	\label{eq:link}
\end{eqnarray} 

% \subsection{Network throughput}

% In order to illustrate the impact of eISL on network throughput, we define the throughput as follows based on \cite{del2019technical,pachler2021updated}:
% \begin{itemize}
% 	\item[1)] Randomly initialize an end-to-end sequence formulated as (source, destination)
% 	\item[2)] Obtain each end-to-end path by the routing algorithm ensuring that there is no two paths share a data link, i.e., the each path can not share common edge between them.
% 	\item[3)] Calculate the bottleneck bandwidth of each path as the throughput of the source satellite.
% 	\item[4)] Calculate the average throughput of the source satellite and sum it as the total throughput of the network.
% \end{itemize}

\subsection{Path stretch and reachable ratio}
The path stretch of a routing algorithm is used to defined as the maximum ratio between the length of any path returned by the algorithm and the length of the shortest path between the same two nodes. In satellite networks, we define the stretch as the ratio of the path propagation distance $L_{prop}$ and the geodesic distance $L_{geo}$ between the same satellites pairs\cite{bhattacherjee2019network}, which is expressed as $stretch = L_{prop}/L_{geo}$.
Since the propagation speed of signal in an optical fiber is about $2c/3$ where $c$ is the speed of light, it can be concluded that if the $stretch \leq 1.5$, the path propagation latency in satellite network is lower than the terrestrial fiber.

% \noindent\textbf{Reachable ratio}
% \subsection{Reachable ratio}

Different with methods \cite{soret2019inter,leyva2021inter} that maximize the total capacity of each ISL,
our main purpose is to allow geographical routing with lower complexity successful applied in satellite networks.
More specifically, we try to use eISL to overcome the 'dead-end' in geographical routing\cite{henderson2000distributed}. 
We define the reachability of path $p^t_i$ under topology $\mathbf{M}_*^t$ at time $t$ as follows:
\begin{eqnarray}
	\mathop{Reach} (p_i^t,\mathbf{M}_*^t)=\left\{
		\begin{aligned}
		1& , & \text{if}~ min\{|\mathbf{M}_*^t - p_i^t| \} \geq 0 \\
		0 & , &\text{else.}
		\end{aligned}
		\right.
\end{eqnarray}
where $p_i^t$ is a routing path, represented as an adjacency matrix and generated by the routing algorithm at time $t$.
Besides, we define the matching problem by maximizing the reachable ratio of paths as follows:
\begin{eqnarray}
	\text{maximize} ~~~ \frac{1}{\|\mathcal{P}\|\|\mathcal{S}\|^2}\sum_{p_i \in  \mathcal{P}}\sum_{\{s_i,s_j\} \subseteq \mathcal{S} } \mathop{Reach} (p^t_i,\mathbf{M}_*^t)
	\label{eq:max}
\end{eqnarray}
where $\|\mathcal{S}\|$ is the number of satellites and $\|\mathcal{P}\|$ is the number of paths generated by routing algorithm.
With $\|\mathcal{S}\|^2$ possible pairs, the complexity of above equation will be $O(\|\mathcal{P}\|\|\mathcal{S}\|^2)$ which is hard to optimize.
In order to address this problem, we propose DeC, a distributed algorithm for matching the encountering satellites that achieves near-optimal solution.
% 目标函数具有较大的复杂度，为
% \noindent\textbf{Stretch}
% \begin{eqnarray}
% 	\frac{1}{\|\mathcal{T}\|} \sum|m_{ij}^t - m^{t-1}_{ij}| 
% \end{eqnarray}


\subsection{Network throughput}
In order to illustrate the impact of eISL on network throughput, we refer \cite{del2019technical,pachler2021updated} and define the throughput but neglecting the ground demands, which as follows:
\begin{itemize}
	\item[1)] Randomly initialize an end-to-end sequence formulated as (source, destination)
	\item[2)] Get each end-to-end path by the routing algorithm and constrain that there is no common edge between each path, i.e., the paths do not share a data link with each other.
	\item[3)] Calculate the bottleneck bandwidth of each path as the throughput of the source satellite.
	\item[4)] Calculate the average throughput of the source satellite and sum it as the system throughput.
\end{itemize}



==> tab/ISLs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
	\caption{Types of Link in space network.}
	\centering
	\scalebox{0.96}{
		\begin{tabular}{|ccc|c|c|c|}
			\hline
			\multicolumn{3}{|c|}{\multirow{2}{*}{Types of Link}}                        & \multirow{2}{*}{Connected Entities}                             & \multirow{2}{*}{Dynamic}  & \multicolumn{1}{l|}{\multirow{2}{*}{At Edge}}                       \\
			\multicolumn{3}{|c|}{}                                                     &                                                                 &                           & \multicolumn{1}{l|}{}                                               \\ \hline
			\multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Inter Satellite Link\\ (ISL)\end{tabular}}}           & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Persistent\\ ISL\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}intra-orbit ISL\\ (iISL)\end{tabular} & adjacent satellites in same orbit             & \faTimes & \faTimes \\ \cline{3-4}
			\multicolumn{1}{|c|}{}                                                     & \multicolumn{1}{c|}{}                                           & \begin{tabular}[c]{@{}c@{}}Inter-orbit ISL\\ (sISL)\end{tabular} & satellites in adjacent orbits                 & \faTimes & \faTimes \\ \cline{2-4}
			\multicolumn{1}{|c|}{}                                                     & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Temporary\\ ISL\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}Encounter ISL\\ (eISL)\end{tabular} & satellites in crossed orbits                          & \faCheck & \faTimes \\ \cline{3-4}
			\multicolumn{1}{|c|}{}                                                     & \multicolumn{1}{c|}{}                                           & \begin{tabular}[c]{@{}c@{}}Inter-shell ISL\\ (oISL)\end{tabular} & satellites in adjacent shells                  & \faCheck & \faTimes \\ \cline{1-4}
			\multicolumn{3}{|c|}{\multirow{4}{*}{Ground station satellite link (GSL)}} & \multirow{2}{*}{NGEO satellite and ground station}              & \multirow{2}{*}{\faCheck} & \multirow{2}{*}{\faCheck}                                           \\
			\multicolumn{3}{|c|}{}                                                     &                                                                 &                           &                                                                     \\ \cline{4-4}
			\multicolumn{3}{|c|}{}                                                     & \multirow{2}{*}{GEO satellite and ground station}               & \multirow{2}{*}{\faTimes} & \multirow{2}{*}{\faTimes}                                           \\
			\multicolumn{3}{|c|}{}                                                     &                                                                 &                           &                                                                     \\ \cline{1-4}
			
			\multicolumn{3}{|c|}{\multirow{2}{*}{Mobile station satellite link (MSL)}} & \multirow{2}{*}{satellite and mobile station}                   & \multirow{2}{*}{\faCheck} & \multirow{2}{*}{\faCheck}                                           \\
			\multicolumn{3}{|c|}{}                                                     &                                                                 &                           &                                                                     \\ \hline
		\end{tabular}
	}
	\label{tab:ISL}
\end{table*}

==> tab/mses.tex <==
\begin{table*}[]
	\caption{Detailed information of mobile stations.}
	\label{tab:acs}
	\centering
	\scalebox{0.96}{
		\begin{tabular}{c|ccccccccccc}
			\toprule[2pt]
			\vspace{2pt}
			station Name        & AC00     & AC01     & AC02     & AC03     & AC04     & AC05     & AC06     & AC07     & AC08     & AC09     & AC10     \\ \hline

			Start Point     & 0E,50N   & 18E,50N  & 36E,50N  & 54E,50N  & 72E,50N  & 90E,50N  & 0E,40N   & 0E,30N   & 0E,20N   & 0E,10N   & 0E,0N    \\
			End Point       & 180W,50S & 162W,50S & 144W,50S & 126W,50S & 108W,50S & 90E,50S  & 180W,40S & 180W,30S & 180W,20S & 180W,10S & 180W,0S  \\
			Distance (km)   & 19998.15 & 17461.25 & 15062.56 & 13020.83 & 11599.87 & 11081.69 & 19970.32 & 19972.31 & 19977.69 & 19984.97 & 19992.30 \\
			Velocity (km/s) & 10.1     & 8.81     & 7.60     & 6.57     & 5.85     & 5.59     & 10.08    & 10.08    & 10.08    & 10.08    & 10.08    \\
			\toprule[2pt]
			% \multicolumn{8}{l}{\small $\bullet$ denotes the Distance of LER moving instead of end-to-end distance.}                         \\
		\end{tabular}
	}

\end{table*}

==> tab/parameters.tex <==
\begin{table}[t!]
	\caption{PARAMETER SETTINGS FOR PERFORMANCE EVALUATION}
	\centering
	\scalebox{0.96}{
		\begin{tabular}{lll}
			\toprule[2pt]
			Parameter          & Symbol    & Setting  \\  \toprule[1pt]
			Number of total satellites & $N$ & 400  \\
			Number of orbital planes & $P$ & 20 \\
			Number of satellites per orbital plane & $N_P$ & 20 \\
			% Avg. length of ISL (without eISL) && 2009km\\
			Satellite altitude&$h$&550km\\
			Inclination of the orbital planes &$\delta$  & $53^\circ$ \\
			Constellation phase factor&$F$& 0\\
		
			% \hline
			Equivalent isotropically radiated power&  ERIP& $31 dBW$ \\
			System bandwidth &$B$&1 GHz\\
			Carrier frequency &$f$&12 GHz\\
			Noise temperature &$T_s$& 324.81K\\

			Access duration threshold &$T_\delta$ & 80 s\\
			Topological distance threshold &$g_\delta$& $\{2,4,6,8\}$\\
		

			\toprule[2pt]
		\end{tabular}

	}
	\label{tab:param}

\end{table}
